Investigating Youth AI Auditing

Youth are active users and stakeholders of artificial intelligence (AI), yet they are often not included in responsible AI (RAI) practices. Emerging efforts in RAI largely focus on adult populations, missing an opportunity to get unique perspectives of youth. This study explores the potential of youth (teens under the age of 18) to engage meaningfully in RAI, specifically through AI auditing. In a workshop study with 17 teens, we investigated how youth can actively identify problematic behaviors in youth-relevant ubiquitous AI (text-to-image generative AI, autocompletion in search bar, image search) and the impacts of supporting AI auditing with critical AI literacy scaffolding with guided discussion about AI ethics and an auditing tool. We found that youth can contribute quality insights, shaped by their expertise (e.g., hobbies and passions), lived experiences (e.g., social identities), and age-related knowledge (e.g., understanding of fast-moving trends). We discuss how empowering youth in AI auditing can result in more responsible AI, support their learning through doing, and lead to implications for including youth in various participatory RAI processes.

==> content/abstract.tex <==
\begin{abstract}
In recent years, there has been a growing recognition of the need to incorporate lay-people's inputs into the governance and acceptability assessment of AI usage. 
% Despite this acknowledgment, we still lack a thorough understanding of the attitudes and reasoning factors that influence people's decisions regarding AI's development and integration. 
However, how and why people judge various AI use cases as acceptable remains under-explored.
In this work, we investigate the attitudes and reasoning factors that influence people's decisions regarding AI's development and integration, via 
% Therefore, our study aims to investigate these dimensions by conducting 
a set of surveys with demographically diverse participants (N=397). 
We focus on ten different AI use cases in both professional (e.g., Lawyer AI) and personal (e.g., Digital Medical Advice AI) settings, to understand the nature and stakes level of use cases on acceptability. 
We further explore the impact of various factors, such as the intervention of engaging participants with explicit considerations of harms and benefits, along with demographic influences, on the judgment of AI use cases.
Moreover, we explore the effects of various types (e.g., cost-benefit reasoning, rule-based reasoning) and factors (e.g., moral values) of decision-making in participants' judgment rationales. 
Our findings indicate that personal use cases are generally perceived more positively and with less disagreement compared to labor-focused ones. 
This study initiates uncovering diverse perspectives that influence societal AI decisions, helping align its development with public expectations and concerns.
% \maarten{I'm wondering if we wanna mirror some more of the intro framing, particularly around the points that (1) we need more democratic/lay people input into AI governance/acceptability of AI, but (2) we don't really know what attitudes and reasoning factors affect people's decisions. Thus, we conduct...
% (I don't think we need to mention dilemmas here, unless we have a paper title that contains the words dilemmas)}
% As AI's capabilities expand, it presents numerous dilemmas stemming from its dual positive and negative impacts. However, we do not yet understand how people with various backgrounds make these decisions, which could provide insights into potential disagreements around AI and possible solutions. 
% As a first step towards understanding the reasoning process regarding AI dilemmas, we construct two studies to understand the effects of use cases (e.g., Lawyer AI, Digital Medical Advice AI), explicit reasoning and various reasoning factors such as moral values and reasoning type (e.g., cost-benefit, rule-based), and demographic factors. We conduct our studies with N=198 and N=199 demographically diverse participants and found that personal use cases were more positively perceived with less disagreements compared to labor related use cases. \jimin{talk more about some coherent findings here and our discussion points}
\end{abstract}

==> content/discussion.tex <==
\section{Discussion}
\jimin{
- moral dilemma in use cases? disagreement between develop / not develop, which are moral dilemmas? how can we know which are
- reasoning patterns that are prevelant tools to support reasoning, especially cost to whom and benefit to whom
- for those that are dilemmas what are the ways people want mitigation, for example, is it context dependent or trust dependent and what kinds of mitigations are possible and from whom?
- people factors, gender divide around healthcare
- use case factors, so something about whether education / ai risk levels are reflective and what does that mean for law-makers?
- empathy, some roles that expect empathy}

\wesley{Maybe also: - Channeling insights from understanding lay users to AI developers and researchers to close the loop. (can help write a subsection if we think this would be a good discussion point).}

==> content/findings.tex <==
% KEY TAKEAWAYS
% RQ1. 
% 1. Some use cases are more acceptable than others
% 2. Some use cases have bigger disagreement
% - good TODO correlation between stake level and standard deviation / confidence
% 3. TODO we need something with confidence
% RQ2: Reasoning effect
% 1. Weighing harms and benefits seemingly no effect on existence in aggregate - confirming related work or not?
% 2. Near significant effect of reasoning on usage acceptability in aggregate - positive
% Check paired t-test
\section{Findings}
\input{tables/use-case-effect}
% \input{figures/decisions_by_use_case}
\input{figures/judgments_by_use_case_violin}
\input{tables/use-case-effects-sd}
\subsection{RQ1. Use Case Factors}
\jimin{sub RQs: 1) main effect, 2) disagreement -- discuss graph (TODO)}
We carefully chose and varied the use cases and analyzed the decisions of existence and usage of the applications to understand the differences between a wide range of use cases. As shown in Table~\ref{table:use-case-effect}, we found a statistically significant relationship between the two categories with jobs having a negative coefficient, on both decisions about existence ($-0.29$, $p<.001$) and usage ($-0.18$, $p<.01$) for the decisions about usage, and personal use cases having a positive coefficient for both decisions as well ($0.60$, $p<.001$; $0.37$, $p<.001$). 

Within the labor replacement use cases, Telemarketer AI ($-0.22$, $p<.05$) and Elementary School Teacher AI ($-0.57$, $p<.001$) had negative coefficients that were statistically significant to decisions on existence. Surprisingly, only one use case, IT Support Specialist AI, had a positive coefficient ($0.49$, $p<.001$) for existence but for usage, both IT Support Specialist AI ($0.94$, $p<.001$) and Government Eligibility Interviewer AI ($0.32$, $p<.01$) had positive coefficients. Unlike the labor replacement use cases, personal use cases showed a decreasing pattern following the variation of EU AI risk levels. Both high risk and high / limited risk use cases, Digital Medical Advice AI ($-0.52$, $p<.001$; $-0.38$, $p<.001$) and Customized Lifestyle Coach AI ($-0.23$, $p<.05$; $-0.21$, $p<.05$), respectively, had negative coefficients for both existence and usage. Similarly, Flavorful Swaps AI, which reflects low risk level had positive coefficients for both existence and usage ($0.45$, $p<.001$; $0.29$, $p<.01$). 

\input{tables/reasoning-main-effects}
% \input{figures/reasoning_within_mean_graphs}
% \input{tables/reasoning-effect-interaction}
\input{tables/reasoning-effects-by-use-case}
\subsection{RQ2. Reasoning Effect}
\jimin{sub RQs: 1) main effect, 2) interaction - use case and reasoning effect. Note - discuss graph}
First, to understand the possible impact of weighing harms and benefits of the use case on participants' decisions, we analyzed the effect of participant's answers before and after the explicit harms and benefits reasoning (Study 2; see \S~\ref{sssec:survey-qs} for details). We first analyzed the main effect, without considering the variations due to the use cases, by fitting a linear mixed effects model, \texttt{Judgment ~ measurementTime + (1|Subject)}, where we create two models with \texttt{Judgment} defined as either standardized value of existence multiplied by confidence or usage multiplied by confidence. As shown in Table~\ref{table:reasoning-effects-main}, only usage judgment after weighing harms and benefits had a marginally significant positive coefficient ($0.06$, $p<.1$). Similarly, for \textbf{Exist$\times$Conf.}, there was no significant effect of \texttt{measurmentTime} on the outcome at the \( p < 0.05 \) level, \( F(1, 200.78) = 0.52, p = 0.4717 \) when analyzed with ANOVA. For \textbf{Usage$\times$Conf.}, there was a marginally significant effect of \texttt{measurementTime} on the outcome at the \( p < 0.1 \) level, \( F(1, 201.05) = 3.37, p = 0.068 \). Surprisingly, when considering the interaction between \texttt{useCase} and \texttt{measurementTime}, only Customized Lifestyle Coach AI had a significant negative coefficient ($-0.31, p<.05$) as shown in Table~\ref{tab:reasoning-effect-interaction}. 

\input{tables/reasoning-factors-questionnaires-effects}
\subsection{RQ3. Reasoning Factors}
\jimin{subRQs: 1) reasoning characteristics of participants and judgment, 2) use case x reasoning factors 
(Study 1), 3) reasoning factors (in written response) x questionnaire factors -- is the questionnaire predictive of the moral values used in the reasoning step?, 4) reasoning factors (in written response) x use case effects on judgment?, 5) reasoning factors (in written response) x reasoning type -- are there specific moral values that are more common in different types of reasoning?

TODO: separate into paragraphs}
We annotated and analyzed open-text reasoning responses as well as responses to questionnaires (MFQ, Toronto Empathy Questionnaire, Oxford Utilitarianism Scale) to understand both contextually specific and general reasoning patterns and their effects on judgments of AI use cases. 

\subsection{Questionnaires}
Interestingly, only Loyalty had a significant effect on both existence ($0.20, p<.001$) and usage ($0.20, p<.01$) as shown in Table~\ref{tab:reasoning-factors-questionnaires}. Moreover, Empathy had a positive and marginally significant effect for usage ($.09, p<.1$). However, Loyalty, as shown in Figure~\ref{fig:moral_values_proportions} and Table~\ref{tab:chi_squared_results}, does not appear as frequently in participants' open text responses compared to values such as Care and Fairness and is the only value that did not have a significant association with use cases. 
\jimin{TODO: correlations between questionnaire values -- e.g., is care for example highly correlated with empathy?}

\input{figures/reasoning_type_by_use_cases}
\input{tables/reasoning-factor-use-case-moral-chi}
\input{figures/moral_values_proportions}
\input{tables/reasoning-factors-moral-values-annotations}
\subsection{Open-text Reasoning Annotations}
\paragraph{Reasoning Type}
\paragraph{Moral Values}
\paragraph{Primary Concern}

\subsection{RQ4. Demographic Factors}
